Training Tensor Attention Efficiently: From Cubic to Almost Linear Time

Tensor Attention, a multi-view attention that is able to capture high-order correlations among multiple modalities, can overcome the representational limitations of classical matrix attention. However, the $O(n^3)$ time complexity of tensor attention poses a significant obstacle to its utilization in transformers, where $n$ is the input sequence length. In this work, we prove that the backward gradient of tensor attention training can be computed in almost linear time $n^{1+o(1)}$, the same complexity as its forward computation under the bounded entries assumption. We provide a closed-form solution for the gradient and propose a fast computation method utilizing polynomial approximation methods and tensor algebraic techniques. Furthermore, we prove the necessity and tightness of our assumption through hardness analysis, showing that slightly weakening it renders the gradient problem unsolvable in truly subcubic time. Our theoretical results establish the feasibility of efficient higher-order transformer training and may facilitate practical applications of tensor attention architectures.

==> 59_impact.tex <==
\section{Impact Statement} \label{sec:impact}

We delve into and offer a deeper understanding of the attention mechanism, introducing a novel approach to integrate multi-modality into attention through the tensor attention algorithm. We also demonstrate that the computation of both forward and backward tensor attention can be achieved with almost linear time complexity. 
Regarding the negative societal impact, since our work is theoretical in nature, we do not foresee any potential negative societal impacts which worth pointing out.
